Towards Efficient Controller Synthesis Techniques for Logical LTL Games

Two-player games are a fruitful way to represent and reason about several important synthesis tasks. These tasks include controller synthesis (where one asks for a controller for a given plant such that the controlled plant satisfies a given temporal specification), program repair (setting values of variables to avoid exceptions), and synchronization synthesis (adding lock/unlock statements in multi-threaded programs to satisfy safety assertions). In all these applications, a solution directly corresponds to a winning strategy for one of the players in the induced game. In turn, \emph{logically-specified} games offer a powerful way to model these tasks for large or infinite-state systems. Much of the techniques proposed for solving such games typically rely on abstraction-refinement or template-based solutions. In this paper, we show how to apply classical fixpoint algorithms, that have hitherto been used in explicit, finite-state, settings, to a symbolic logical setting. We implement our techniques in a tool called GenSys-LTL and show that they are not only effective in synthesizing valid controllers for a variety of challenging benchmarks from the literature, but often compute maximal winning regions and maximally-permissive controllers. We achieve \textbf{46.38X speed-up} over the state of the art and also scale well for non-trivial LTL specifications.

==> complete-approach.tex <==
\section{Complete Approach - GenSys-LTL}

\DD{Superceded?}

  
Algorithm \ref{proc: gensys-ltl} shows the high-level description of our approach. Our approach takes as input a game specification in the form of $Con(V, V')$ and $Env(V, V')$ over the variables $V$.  These transition relations induces a two player alternating infinite game over the concrete valuations over $V$. It also takes as input the winning condition in the form of an LTL specification $Spec_{LTL}(V)$ over $V$. If the procedure terminates, it gives the winning region + strategy as the output or admits unrealizability.
 
\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $Spec_{LTL}(V)$}
\Output{ Winning Region, Unrealizable, Timeout}

\If {$Spec_{LTL}(V) \ \in \ \{ G(\phi(V)) , \ F(\phi(V)), \ GF(\phi(V)), \ FG(\phi(V)) \} $ }{
    \Comment{GenSys with predicate specs}
    \Return $GenSys(Con, Env,  \phi(V))$;
}
\Else{
    $Aut(q, V, q'),  F(q)$ := $LTL2BA(Spec_{LTL}(V))$;
    
    \If{isDeterministic(Aut)}{
        \Return $Buchi\_FixedPoint(Con, Env, Aut, F)$;
    }
    \Else{
         $Aut\_(q, V, q'),  F\_(q)$ := $LTL2BA( \neg Spec_{LTL}(V))$;

        \If{isDeterministic(Aut\_)}{
        \Return $CoBuchi\_FixedPoint(Con, Env, Aut\_, \neg F)$;
        }
        \Else {
            \Comment{OTF or Antichain approaches}
            k = 0;
            
            \Do{$W_1$ = $W_2$}{
            		 $W_1$ := $K\_FixedPoint(Con, Env, Aut\_,F\_, k)$;
            		 
            		  $W_2$ := $K\_FixedPoint(Env,  Con,Aut, F, k)$;
            		  
            		  k++;
            }
            
            \Return ($W_1$, k);
        }
    }
}
\caption{GenSys-LTL approach overview}
\label{proc: gensys-ltl}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{LTL Formula $Spec_{LTL}(V)$}
\Output{Buchi Automaton $Aut(q, V, q')$}

1. Replace atomic predicates of $Spec_{LTL}(V)$ with Boolean propositions $P$.  Store this in a map $M: atoms(V) \rightarrow P$

2. Use the resulting propositional LTL formula to generate a propositional Buchi Automata $Aut(q, P, q')$.
 
3. Replace propositions with predicates using $M$ to get $Aut(q, V, q')$.

4.  \Return $Aut(q, V, q')$

\caption{LTL to Buchi Automata conversion}
\label{proc: ltl2ba}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{$Aut(q, V, q')$}
\Output{Yes/ No}

\Comment{To Sir: s is a concrete valuation of V,  as defined in the first page.}

\If{ $\forall q, s. |Aut(q,  s) | == 1$ }{\Return Yes}
\Else{\Return No}

\caption{Algorithm to check if a given Buchi Automaton is deterministic}
\label{proc: isdeterministic}
\end{algorithm}


Lines 1-2 checks if $Spec_LTL(V)$ is in one of the forms $G(\phi(V))$ ,$ F(\phi(V))$, $GF(\phi(V))$,  or $FG(\phi(V)) $.  If yes,  it falls back to the non-LTL version of GenSys which uses traditional fixed-point procedures over the predicate specifications. It should be noted that these formulas do not have nested temporal operators.  Algorithms \ref{proc: gensys-safety}, \ref{proc: gensys-reachability},  \ref{proc: gensys-buchi}, and \ref{proc: gensys-cobuchi} explain these 4 approaches corresponding to the temporal operators $G$ , $F$, $GF$, and  $FG$ respectively.  Lines 4-10 focuses on the cases where the specification is a generic LTL formula where either the specification or it's negation generates a deterministic Buchi automaton using any standard LTL to Buchi Automaton conversion approach.  Algorithm \ref{proc: ltl2ba} explains our approach for the same.  Note that we require a complete automaton for our approach (i.e., from a given state $q$ and a concrete valuation $s$ over $V$,  a target state $q'$ must exist ).  Next, we check if the resulting Buchi automata $Aut$ is deterministic using the condition in Algorithm \ref{proc: isdeterministic}.  If the spec generates a deterministic Buchi Automata, we use the $Buchi\_FixedPoint$ (Algorithm \ref{proc: gensys-buchi-aut}) approach that asks for a strategy for $Con$ player to win the game with a Buchi condition over the final states $F$.  If the negation of the spec generates a deterministic Buchi Automata, we use the $CoBuchi\_FixedPoint$ approach (Algorithm \ref{proc: gensys-cobuchi-aut}) that asks for a strategy for the $Con$ player to win the game with the CoBuchi condition over $\neg F$.  In the resulting product game,  $F$ essentially becomes the set of all product states such that the automaton component of the product state is a final state of the automaton.  in these two algorithms is the set o Lines 11-18 focus on the cases where neither automatons are deterministic.  In such a case, we use the non-deterministic automaton generated by the negation of the specification. We apply the Universal Co-Buchi condition to it which enables us to reduce the game to a k-bounded safety game.  We then solve this game using one of the two in $K\_FixedPoint$ approaches; they are the On-The-Fly Determinization approach and an Antichain Based Approach.  Essentially,  we check for a given $k$,  whether the controller can ensure $Spec_{LTL}(V)$ or whether the environment  can ensure $\neg Spec_{LTL}(V)$.  If the winning region for the controller for $Spec_{LTL}(V)$ is $W$,  for every $k$, the controller returns an underapproximation $W_1 \implies W$ and the  environment returns an overapproximation $W \implies W_2$. We terminate if both are equal.  Sections \ref{sec:otf} and \ref{sec:antichain} explain these two k-fixedpoint approaches in detail.

It must be noted that the complexity of solving the problem increases as we move from lines 1 to 12. This is because the predicate-based approach (Lines 1-2) is much simpler conceptually and in terms of formula size as compared to the deterministic Automaton-based approaches (Lines 4-10). The Bounded  K-Fixed-point approaches (Lines 11-18) deal with complex constraints for handling determinism and antichains, apart from iterating over a bounded range. This makes them the most complex from an SMT solver's perspective. \textbf{The research question is to empirically understand how often we reach this case and how well we perform compared to other state-of-the-art tools.}

At the heart of GenSys, all the above approaches rely on four fundamental fixed-point techniques from the literature: 

\[
\square: \nu X. \  (\wpr_S(X)  \wedge  G)
\]

\[
\lozenge: \mu X. \  (\wpr_R(X)  \vee  G)
\]

\[
\lozenge \square: \mu W \nu H. \  (\wpr(H) \wedge (\wpr(W)  \vee  G)
\]

\[
\square \lozenge: \nu W \mu H. \  (\wpr(H) \vee (\wpr(W)  \wedge  G)
\]x

The definitions of $\wpr$ and $G$ change with each approach based on whether predicates, automatons, or determinized automatons are used. For example, if we use predicates, then $G$ would be $G(V)$ (i.e., the non-temporal predicate formula), and $\wpr_S(X)$, $\wpr_R(X)$ and $\wpr(X)$ are defined as follows:

$$
\begin{array}{lcl}
\wpr_S(X)& \equiv & \exists V' (Con(V,V') \ \wedge G(V') \ \wedge\\
&& \ \forall V'' (
Env(V', V'') \implies  X(V''))).
\end{array}
$$

 $$
 \begin{array}{lcl}
 \wpr_R(X)& \equiv & \exists V' (Con(V,V') \ \wedge (G(V') \ \vee\\
 && \ \forall V'' (
 Env(V', V'') \implies  X(V'')))).
 \end{array}
 $$
 
$$
\begin{array}{lcl}
\wpr(X)& \equiv & \exists V' (Con(V,V') \ \wedge \\
&& \ \forall V'' (
Env(V', V'') \implies  X(V''))).
\end{array}
$$

If we are solving a product game with a deterministic Buchi automaton $Aut(q, V, q')$,  then $G$ would be $F(q)$ (final states of the automaton $Aut$) and $\wpr$ would be $\wpr_A$ as follows: 

$$
\begin{array}{lcl}
\wpr_A(X)& \equiv & \exists V', q' (Con(V,V') \ \wedge \ Aut(q, V, q') \\
&& \ \forall V'', q'' (
(Env(V', V'') \ \wedge \ Aut(q,' V, q'') \ ) \implies  X(V'', q''))).
\end{array}
$$


\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $G(V)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}

$W_0$ := $W_1$ := G;

\Do{$W_0 \nRightarrow W_1$}{ 
$W_0$ := $W_1$; 

$W_1$ := $\wpr_S(W_0) \wedge G$

}

\Return $W_0$;

\caption{Safety Fixed-Point Procedure - GenSys}
\label{proc: gensys-safe}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $G(V)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}

$W_0$ := $W_1$ := G;

\Do{$W_1 \nRightarrow W_0$}{ 
$W_0$ := $W_1$; 

$W_1$ := $\wpr_R(W_0) \vee G$

}

\Return $W_0$;

\caption{Reachability Fixed-Point Procedure - GenSys}
\label{proc: gensys-reachability}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $G(V)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}

$W_0$ := $W_1$ := True;

\Do{$W_0 \nRightarrow W_1$}{ 
$W_0$ := $W_1$; 

$H_0$ := $H_1$ := False;

    \Do{$H_1 \nRightarrow H_0$}{ 
    $H_0$ := $H_1$; 

    $H_1$ :=  $\wpr(H_0) \vee (\wpr(W_0) \wedge G)$

    }

$W_1$ := $H_0$;

}

\Return $W_0$;

\caption{Buchi Fixed-Point Procedure - GenSys}
\label{proc: gensys-buchi}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $G(V)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}

$W_0$ := $W_1$ := False;

\Do{$W_1 \nRightarrow W_0$}{ 
$W_0$ := $W_1$; 

$H_0$ := $H_1$ := True;

    \Do{$H_0 \nRightarrow H_1$}{ 
    $H_0$ := $H_1$; 

    $H_1$ :=  $\wpr(H_0) \wedge (\wpr(W_0) \vee G)$

    }

$W_1$ := $H_0$;

}

\Return $W_0$;

\caption{CoBuchi Fixed-Point Procedure - GenSys}
\label{proc: gensys-cobuchi}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $Aut(q, V, q')$, $F(q)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}
\Comment{W and H are formulae over (V,q).  }

$W_0$ := $W_1$ := True;

\Do{$W_0 \nRightarrow W_1$}{ 
$W_0$ := $W_1$; 

$H_0$ := $H_1$ := False;

    \Do{$H_1 \nRightarrow H_0$}{ 
    $H_0$ := $H_1$; 

    $H_1$ :=  $\wpr_A(H_0) \vee (\wpr_A(W_0) \wedge F)$

    }

$W_1$ := $H_0$;

}

\Return $W_0$;

\caption{Buchi Fixed-Point Procedure with Deterministic Automaton}
\label{proc: gensys-buchi-aut}
\end{algorithm}

\begin{algorithm}
% \SetAlgoLined
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwRepeat{Do}{do}{while}
\Input{ $Con(V, V')$, $Env(V, V')$, $Aut(q, V, q')$, $F(q)$}
\Output{ Realizable+Strategy, Unrealizable, Timeout}
\Comment{W and H are formulae over (V,q).  }

$W_0$ := $W_1$ := False;

\Do{$W_1 \nRightarrow W_0$}{ 
$W_0$ := $W_1$; 

$H_0$ := $H_1$ := True;

    \Do{$H_0 \nRightarrow H_1$}{ 
    $H_0$ := $H_1$; 

    $H_1$ :=  $\wpr_A(H_0) \wedge (\wpr_A(W_0) \vee F)$

    }

$W_1$ := $H_0$;

}

\Return $W_0$;

\caption{Co-Buchi Fixed-Point Procedure with Deterministic Automaton}
\label{proc: gensys-cobuchi-aut}
\end{algorithm}


==> games-old.tex <==
\section{Logical Games (Old)}

In this section, we introduce our game model and the specification semantics. We focus on a two-player, alternating logical game that must satisfy a temporal specification; this specification can be internally or externally specified. The game has both functional and reactive components. The functional component is a stateless update over the game states whereas the reactive component enforces a temporal restriction over these concrete valuations of game states. The controller synthesized for this synthesis problem ensures that the game states are updated in a manner such that the temporal specification is satisfied.

\subsection{Game}
We consider two-player games played between player 0 and player 1.  We call player 0 as the controller and player 1 as the environment.  
A game consists of a game graph $G$ and a winning condition .  The (rules of the) game graph are specified using predicates over the player moves whereas the winning condition can be specified using temporal logic over predicates or automatons over predicates.  We explain each component below.

\subsubsection*{Game Graph:} The rules of the game are specified by the allowable moves of controller and environment.  These moves are described using the predicates $\envi(V,V')$,  and $\cont(V,V')$ respectively,  over the set of game variables $V$,  as defined in GenSys \cite{} \footnote{Please note that we now denote $V$ to denote the set of game variables,  $S$ to denote the set of concrete game states,  and $Q$ to denote states of the property automaton, unlike GenSys where we used $S$ to denote variables}.  We consider these predicates to be in the quantifier free fragment of first order logic with the theory of linear integer arithmetic.  

Let $G$ be a concrete game graph induced by the moves above.   We define it as follows: $G = \{ S_0,  S_1,  T_C, T_E\}$ where  $S_0 = S_1 = \{ s\ |\ s: V \rightarrow \mathbb{Z}\}$ and $S_0$ (resp. $S_1$) denote the states from which player 0 or the controller (resp.  player 1 or the environment) can make a move.  $T_C$ and $T_E$ are edges in $G$ induced by $\cont(V,V')$,  and $\envi(V,V')$  respectively.  $T_C \subseteq S_0 \times S_1$ such that $ \forall (s,s') \in T_C, v \in V,. \cont(s(v), s'(v))$ is true.  Similarly,  $T_E \subseteq S_0 \times S_1$ such that $ \forall (s,s') \in T_E,  v \in V,. \envi(s(v), s'(v))$ is true.  Thus,  $G$ is a bipartite graph.  Since the domain of $V$ is integers,  the state space of $G$ is infinite and hence we have an infinite concrete game graph.

The above definition of a $G$ allows the controller moves to be non deterministic and infinitely many.  For our setting, we restrict the number of moves of the controller to be finite and also require that each such move is deterministic.  More specifically,  for $n$ moves,  we require $\cont(V,V')$ to be defined as:  $\cont(V,V') = \bigvee_{i = 1}^n \cont_i (V,V')$ where each $\cont_i(V,V')$ is deterministic i.e.,  for every $s \in S_0,  s' \in S_1 s'' \in S_1,  v \in V, i \in \{1, ..., n\}. \ \cont_i(s(v),  s'(v)) \ \wedge \ \cont_i(s(v),  s''(v)) \ \implies \ s'(v) = s''(v)$ ,   Thus,  we do not allow expressions such as $x'>y$ for the controller.  Consequently,  $T_C$ is extended as follows: $T_C = \bigcup_{i=1}^n T_{C_{i}}$,  where $T_{C_{i}} : S_0 \rightarrow S_1$ such that $\forall s \in dom(T_{C_{i}}), v \in V,  \cont(s(v), T_{C_{i}}(s)(v))$ is true.

We illustrate the above with an example.  Let $V = \{x,y\}$.  Thus,  $V' = \{x',y'\}$.  Let the number of controller moves $n$ be 2.  Thus,  let $\cont_1(x,y,x',y') = x' == x\  \wedge \  y' == y+1$ and $\cont_2(x,y,x',y') = x' == x - 2\  \wedge \  y' == y$.  $\cont(x,y,x',y')$ is the disjunction of the above two formulae.  Let the environment move be skip.  We denote this by $\envi(x,y,x',y') = x == x' \wedge y== y'$ .  In general, the environment move could be any non deterministic move. The concrete game graph induced by the above moves is illustrated in Fig.~\ref{fig:game}.

\begin{figure}
\includegraphics[scale = 0.3]{figures/game}
\centering
\caption{Concrete game graph induced by the move predicates $\cont(V,V')$,  and $\envi(V,V')$ over $V = \{x,y\}$.}
\label{fig:game}
\end{figure}

The circle states denote all states in $S_0$ and the square states denote all states in $S_1$.  Since the environment moves are skip,  all edges from $S_1$ to $S_0$ lead back to states with the same values for $x$ and $y$.  All edges from $S_0$ to $S_1$ are labelled $1$ or $2$ depending on whether it is a $T_{C_{1}}$  move or a $T_{C_{2}}$ move.  As you can see,  the controller moves are deterministic,  the players alternate as the graph is bipartite and the state space is infinite.  This is an infinite state concrete game graph.  We refer to this as a game graph from here on.

\subsubsection*{Play:} 
A \emph{play} in a game graph $G$ is as follows: A token is placed in some state $s \in S_0 \cup S_1$.  If the state belongs to the controller,  the controller makes a move by choosing one of the $n$ moves to lead into an environment state.  If the state belongs to the environment,  then the environment makes some non deterministic move that leads the game into some controller state.  This results in an sequence of states $s_0, s_1, s_2, ...$ where every alternate state belong to $S_i$ and the rest belong to $S_{1-i}$. 

\begin{figure}
\includegraphics[scale = 0.2]{figures/play}
\centering
\caption{A (partial) play of the game graph.}
\label{fig:play}
\end{figure}

Fig.~\ref{fig:play} illustrates a play in the game graph of
Fig.~\ref{fig:game}.  The token is first placed in state $(x \mapsto
0,  y \mapsto 0,)$ that belongs to the controller.  The controller
plays the concrete move $T_{C_1}$, that is a model of $\cont_1(V,V')$,
to move the token to the environment state $(x \mapsto 0,  y \mapsto
1)$.  The environment state then moves the token to the controller
state respecting $T_E$ and the game continues,  resulting in a
infinite play.

Formally,  a play in a game graph $G$ is an infinite sequence $s_0, s_1, s_2, ...  \in (S_0 \cup S_1)^\omega$ such that forall $i>=0$, $s_i \in S_i$ and $s_{i+1} \in S_{1-i}$.  If the controller plays first,  then $s_0 \in S_0$,  else if environment plays first, then $s_0 \in S_1$.

We denote all the plays in a game graph $G$ as $Plays(G)$ and plays from $G$ starting from state $s \in (S_0 \cup S_1)$ as $Plays(G, s)$.  

\subsubsection*{Strategy:} 

An important notion of a game are that of its strategies.  A strategy essentially guides the movement of the token in the game graph.  In general the choice of a move from a given vertex depends on the play prefix produced so far.  Thus,  a strategy is a function mapping play prefixes to a successor the prefix's last vertex. 

A strategy for player $i \in \{0,1\}$ in a game graph $G$ is a function \[\sigma :(S_0 \cup S_1)^* S_i \mapsto S_{1-i}\]

Without loss of generality,  we can also define the strategy for the controller (i.e.,  player 0) as \[\sigma :(S_0 \cup S_1)^* S_0 \mapsto \{ 1, 2, ..., n\}\] for $n$ moves of the controller.
\\


\subsubsection*{Consistent Play:} A play that adheres to a given strategy is called a consistent strategy.  Formally,  a play $s_0, s_1, s_2, ...$ in a game graph $G$ is consistent with a strategy $\sigma$ for player $i$ in $G$,  if \[\forall n \in \mathbb{N}. \ s_n \in S_i \implies \ s_{n+1} = \sigma(s_0, s_1,  ...,  s_n) \]
Therefore,  it follows that a play is consistent with a strategy $\sigma$ iff every prefix of it is consistent with $\sigma$.
Given a state $s \in (S_0 \cup S_1)$,  the set of all plays that are consistent with $\sigma$ and start with $s$ are defined as $Plays(G, s,\sigma)$. 

\emph{Note:} If we fix some strategy $\sigma$ for the controller from a start state $s$,  then we can get a set of plays $Plays(G, s,\sigma)$ as this strategy determines the choices of the controller only.  However,  if we also fix another strategy $\tau$ for the environment,  then this would result in a unique play $Plays(G, s,\sigma) \cap Plays(G, s,\tau)$.

\subsubsection*{Positional Strategy:} 

The previous definition of a strategy is not suitable for practical purposes due to the infinite size of the strategy.  Thus, we define a weaker notion of a strategy called \textit{positional strategy}.  Formally,  a strategy $\sigma$ for a player $i$ is a positional strategy,  if $\sigma(wv) = \sigma(v)$ for all $w \in (S_0 \cup S_1)^*$ and $v \in S_i$.  A positional strategy for player $i$ is equivalent to a function \[\sigma: S_i \mapsto S_{1-i}\]. 
Without loss of generality,  we can also define the strategy for the controller (i.e.,  player 0) as \[\sigma : S_0 \mapsto \{ 1, 2, ..., n\}\] for $n$ moves of the controller.
a\subsubsection*{Maximal  Strategy:}  A strategy $\sigma_1$ in a game graph $G$ is maximal if and only if for all strategies $\sigma_2$,  $dom(\sigma_1)\ \supseteq \ dom(\sigma_2)$ and for \Stanly{not sure how to say that for all game states $s \in S$, $\sigma_1(s) \supseteq \sigma_2(s)$ without redefining the notion of a positional strategy as map $\sigma : S_0 \mapsto 2^{\{ 1, 2, ..., n\}}$. This map intuitively means that we are able to merge strategies without loss of generality.  Need to think about this.}

\subsubsection*{Game:} 
\label{subsec:game}
A game graph $G$ under a given winning condition $\Phi \subseteq (S_0 \cup S_1)^\omega$ is called a game $\mathcal{G}$ i.e,  $\mathcal{G} = \{ G,  \Phi\}$ .   A play $\rho$ is $winning$ for player 0 or controller iff $\rho \in \Phi$ else it is winning for player 1 or environment.  For example,  consider the winning condition $\Phi = \{ s_0, s_1, s_2, .. \ |\ s_i(x) == 0.  \forall i \geq 0 \}$.  For the game in Fig.~\ref{fig:game}, a winning play $\rho$ for the controller exists starting from the state $(x \mapsto 0,  y \mapsto 1)$ and ensuring that the controller always plays move $1$, as move $1$ and environment do not change the value of $x$.
There are multiple ways of specifying the winning region.  Methods include using predicates,  automatons and temporal logic formulae,  to name a few.  We will look at these in the further sections. For example,  the LTL formula (will define in detail soon) $G( x == 1 \implies F\  x ==3)$ specifies that it is always true that the value of x should eventually be equal to 3 if it is equal to 1.

\subsubsection*{Winning Strategy:} While playing a game,  both players try to ensure a win against any possible move of the environment.  This is formalized by the notion of a winning strategy.  A \textit{strategy} $\sigma$ is winning for player $i$ in a game graph $G$ from state $s \in S_0 \cup S_1$ if every play that is consistent with $\sigma$ and starts in $s$ is winning for player $i$.

\subsubsection*{Winning Region:} 
The set of states from where player $i$ has a winning strategy is called the winning region which we denote as $W_i(\mathcal{G})$.

\emph{Lemma: } $W_0(\mathcal{G}) \cap W_1(\mathcal{G})$ for every game $\mathcal{G}$.

For the game described in \ref{subsec:game},  the controller can win from all states $s \in S_0 \cup S_1$ such that $s(x) = 0$. Thus,  $W_0(\mathcal{G}) = \{s\ |\ s(x) = 0\}$. The winning strategy for the controller ensures that move $1$ is always chosen in order to win against any move of the environment.



==> old-gensys-approach.tex <==


The basic idea is to first check if the given game $\myGame$ is simple, and if
so compute the winning region and strategy using the procedures
outlined in Sec.~\ref{sec:simple-games}.
If $\myGame$ is not simple, we essentially construct a ``product''
game, which is a simple game, which takes the product of the original
game and a \emph{deterministic} automaton for the LTL specification.

It is important to note that we need deterministic automata in this
setting. App.~\ref{sec:need-determinism} details the problem with
using non-deterministic automata for the specifications. \DD{include
  here itself if space permits?}.


The overall approach followed by \gensysltl\ is described in
Alg.~\ref{proc:gensys-ltl}.  The algorithm takes as input an LTL game $\myGame$.  If this game is realizable,  then a solution to this game is the (canonical) winning region $\winreg{C}{\myGame}$ represented symbolically as $W$.  If the algorithm terminates,  we either return an underapproximation $W_L$ or overapproximation $W_U$ of $W$ and the corresponding strategy $\sigma$ for $W_L$.  

\Stanly{Lines in this algorithm starts with 49. Is this how it is supposed to be?}
Lines 49-52 first checks if $\myGame$ is a simple game of the form $\mathcal{H} = (V, D, \cont, \envi,  \psi)$ as described in Section \ref{sec:simple-games}.  If yes,  we solve this game out of the box using the approaches mentioned in that section.   

If not,  then we will have to reduce $\myGame$ to a simple game.  This requires converting the LTL formula $\psi$ into a \emph{B\"uchi} Automaton $\A_{\psi}$, using standard techniques in the literature, which we abstract out using the function $LTL2BA$.  In the rest of the algorithm,  we will be using $\A_{\psi}$ (or $\A_{\neg \psi}$) to solve the game $\myGame$.  In general,  $\A_{\psi}$ need not be deterministic and can be a  \emph{B\"uchi},  \emph{Co-B\"uchi},  \emph{Safety} automation.  We can represent $\A_{\psi}$ symbolically using the predicate $Aut$ which is a constraint over the variables $ V \cup \{ q, q'\} $,  and the predicates $Init$ and $Final$ which are constraints over ${q}$.  The variables $q$ and $q'$ range over a bounded integer domain $D_Q: \{q,q'\} \rightarrow \{0, 1, 2,  |Q|-1\}$ where $|Q|$ is the number of states in $\A_{\psi}$.   $Aut$ constraints the transitions of $\A_{\psi}$ whereas $Init$ and $Final$ specify the initial and final states respectively, of $\A_{\psi}$.

\begin{figure}
\label{fig:ucw_elevator}
\includegraphics[scale = 0.15]{figures/ucw_elevator}
\centering
\caption{Universal \emph{Co-B\"uchi} Automaton $\A_{\neg \psi}$ for the specification $\psi = G(1<=x<=3) \wedge G(F (x==1) \wedge F (x == 2)  \wedge F (x ==3))$ where $V = \{x\}$.}
\end{figure}

An example of a partial encoding $<Aut, Init, Final>$ for a non-deterministic $UCA$ shown in Figure \ref{fig:ucw_elevator} is:

$$
\begin{array}{lcl}
Aut(q,  x,  q') && \equiv (q == 0 \wedge 1 \leq x \leq 3 \wedge q' == 0)\ \vee \\
&& \ \ \ (q == 0 \wedge \ \neg (1 \leq x \leq 3) \  \wedge q' == 1)\ \vee \\
&& \ \ \ (q == 0 \wedge \ 2 \leq x \leq 3 \ \wedge q' == 2) \vee \\
&& \ \ \ (q == 0 \wedge \ (x == 1 \vee x == 3) \ \wedge q' == 3)\ \vee \\
&& \ \ \ (q == 0 \wedge \ 1 \leq x \leq 2 \ \wedge q' == 4)\ \vee \\
&& \ \ \ (q == 1 \wedge q' == 1)\ \vee \\
&& \ \ \ ...
\end{array}
$$

$$
\begin{array}{lcl}
Final(q) && \equiv (q ==  1 \vee q ==2 \vee q ==3 \vee q ==4 )
\end{array}
$$

$$
\begin{array}{lcl}
Init(q) && \equiv (q ==  0 )
\end{array}
$$

Here, the outgoing edges from states $q_0$ and $q_1$ are encoded in $Aut$.
The final states of $\A_{\neg \psi}$ shown by double circles are states $q_1, q_2 , q3, q4$.  The initial state is state $q_0$ and is represented by $Init$.

Lines 55 -61 show the case when the automaton $\A_{\psi}$ is a deterministic \emph{B\"uchi} atuomaton,. In such a case, we can solve the game by taking a product of the automaton with the logical game.  This can be done by conjuncting $Aut$ with each of the player moves.  Thus,  the resulting simple game now becomes:

\[
\mathcal{H} = (V_H, D_H, \cont_H, \envi_H, \Psi),
\]
where
\begin{itemize}
\item $V_H$ := $V \union \{ q\}$ 
\item $D_H$ := $D \union D_Q$
\item $\cont_H$ := $\cont \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$C$
\item $\envi_H$ := $\envi \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$E$
  \item $\Psi$ := $GF(Final)$
\end{itemize}

We can now solve this game using Algorithm \ref{proc: gensys-buchi} mentioned in Section \ref{sec:simple-games}. 

Similarly,  Lines 62 -67 show the case when the automaton $\A_{\neg\psi}$ is a deterministic \emph{Co-B\"uchi} atuomaton.  In such the case the simple game is the same as above,  except for  $\Psi$ := $FG(Final)$.  We can now solve this game using Algorithm \ref{proc: gensys-cobuchi} mentioned in Section \ref{sec:simple-games}. 

In all the approaches mentioned so far in lines 49 - 65,  we always return the canonical winning region $W$, by construction.

Lines 69-81 show the case when both  $\A_{\neg\psi}$ and $\A_{\neg\psi}$ are non-deterministic.  In such a case,  we reduce the problem to solving the product game over a $UCA$ which is determinized to $k-bounded$ safety automaton.  The determinization step requires the subset construction with counters, and is standard in the literature.  
To find a strategy for player $C$,  in lines 70-74, we first determinize $\A_{\neg\psi}$ for a given $k$ to get $\UCW_{\psi}^k$, which is a safety game from where player C can win the game iff the final states are visited atmost $k$ times.   Let $<Aut, Final>$ be the symbolic encoding of $\UCW_{\psi}^k$.  The simple game to solve now becomes:

\[
\mathcal{H} = (V_H, D_H, \cont_H, \envi_H, \Psi),
\]
where
\begin{itemize}
\item $V_H$ := $V \union C$ , where $C = \{ c_0, c_1, . ..  c_{|Q| -1}\}$.
\item $D_H$ := $D \union D_C$ where  $D_C: C \rightarrow \{0, 1, 2,  k+1\}$
\item $\cont_H$ := $\cont \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$C$
\item $\envi_H$ := $\envi \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$E$
  \item $\Psi$ := $G(Final)$
\end{itemize}

We can now solve this game using Algorithm \ref{proc: gensys-safety} mentioned in Section \ref{sec:simple-games}. 

Similarly,  in lines 75 -80, we check if environment has a strategy for $\neg \psi$.  If $<Aut, Final>$ is the symbolic encoding of of $\UCW_{\neg \psi}^k$, then the resulting game is:

\[
\mathcal{H} = (V_H, D_H, \envi_H, \cont_H, \Psi)
\]

where,  the definitions for each entry in the tuple is same as above.

\Stanly {This section needs to be better phrased}
For an increasing value of $k>=0$, we run both environment and controller strategies in parallel,  until $W_L == W_U$ or timeout.

We can now plug in $Con(V, V')$, $Env(V, V')$, and $Aut(q, V, q')$ into one of our two fixedpoint approaches to synthesize a controller to the above solution. Both approaches rely on a conversion from $Aut(q,V,q')$ to a $k$-safety game to check for $k$ realizability. If a solution is not found for a given value of $k$, we search for a higher value of $k$. Moreover, since the game is determined, we can also check for the realizability of $Env(V, V')$ in parallel and stop when one of the two says realizable. The advantage of both our approaches is that we do not determinize to a k-safety automaton manually. We encode constraints that reason over the determinized k-automaton during the fixedpoint computation itself, eliminating the need for explicit determinization. In the second approach, we optimize the first approach by using antichains to represent the state space compactly. In Section \ref{sec:otf}, we introduce the On-The-Fly determinization approach where explicit determinization is avoided and in Section \ref{sec:antichain}, we optimize the OTF approach using antichains to effectively make use of the state space.




\Stanly{Done:
  \begin{itemize}
  \item Describe representing automata symbolically
  \item Describe product game (symbolic)
  \item Describe UCW approach at high-level, refer to next
    sec/sections for details of OTF and Antichains.
  \end{itemize}}


\begin{figure}
\label{fig:ucw_elevator}
\includegraphics[scale = 0.15]{figures/ucw_elevator}
\centering
\caption{Universal \emph{Co-B\"uchi} Automaton $\A_{\neg \psi}$ for the specification $\psi = G(1<=x<=3) \wedge G(F (x==1) \wedge F (x == 2)  \wedge F (x ==3))$ where $V = \{x\}$.}
\end{figure}

An example of a partial encoding $<Aut, Init, Final>$ for a non-deterministic $UCA$ shown in Figure \ref{fig:ucw_elevator} is:

$$
\begin{array}{lcl}
Aut(q,  x,  q') && \equiv (q == 0 \wedge 1 \leq x \leq 3 \wedge q' == 0)\ \vee \\
&& \ \ \ (q == 0 \wedge \ \neg (1 \leq x \leq 3) \  \wedge q' == 1)\ \vee \\
&& \ \ \ (q == 0 \wedge \ 2 \leq x \leq 3 \ \wedge q' == 2) \vee \\
&& \ \ \ (q == 0 \wedge \ (x == 1 \vee x == 3) \ \wedge q' == 3)\ \vee \\
&& \ \ \ (q == 0 \wedge \ 1 \leq x \leq 2 \ \wedge q' == 4)\ \vee \\
&& \ \ \ (q == 1 \wedge q' == 1)\ \vee \\
&& \ \ \ ...
\end{array}
$$

$$
\begin{array}{lcl}
Final(q) && \equiv (q ==  1 \vee q ==2 \vee q ==3 \vee q ==4 )
\end{array}
$$

$$
\begin{array}{lcl}
Init(q) && \equiv (q ==  0 )
\end{array}
$$

Here, the outgoing edges from states $q_0$ and $q_1$ are encoded in $Aut$.
The final states of $\A_{\neg \psi}$ shown by double circles are states $q_1, q_2 , q3, q4$.  The initial state is state $q_0$ and is represented by $Init$.

Lines 55 -61 show the case when the automaton $\A_{\psi}$ is a deterministic \emph{B\"uchi} atuomaton,. In such a case, we can solve the game by taking a product of the automaton with the logical game.  This can be done by conjuncting $Aut$ with each of the player moves.  Thus,  the resulting simple game now becomes:

\[
\mathcal{H} = (V_H, D_H, \cont_H, \envi_H, \Psi),
\]
where
\begin{itemize}
\item $V_H$ := $V \union \{ q\}$ 
\item $D_H$ := $D \union D_Q$
\item $\cont_H$ := $\cont \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$C$
\item $\envi_H$ := $\envi \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$E$
  \item $\Psi$ := $GF(Final)$
\end{itemize}

We can now solve this game using Algorithm \ref{proc: gensys-buchi} mentioned in Section \ref{sec:simple-games}. 

Similarly,  Lines 62 -67 show the case when the automaton $\A_{\neg\psi}$ is a deterministic \emph{Co-B\"uchi} atuomaton.  In such the case the simple game is the same as above,  except for  $\Psi$ := $FG(Final)$.  We can now solve this game using Algorithm \ref{proc: gensys-cobuchi} mentioned in Section \ref{sec:simple-games}. 

In all the approaches mentioned so far in lines 49 - 65,  we always return the canonical winning region $W$, by construction.

Lines 69-81 show the case when both  $\A_{\neg\psi}$ and $\A_{\neg\psi}$ are non-deterministic.  In such a case,  we reduce the problem to solving the product game over a $UCA$ which is determinized to $k-bounded$ safety automaton.  The determinization step requires the subset construction with counters, and is standard in the literature.  
To find a strategy for player $C$,  in lines 70-74, we first determinize $\A_{\neg\psi}$ for a given $k$ to get $\UCW_{\psi}^k$, which is a safety game from where player C can win the game iff the final states are visited atmost $k$ times.   Let $<Aut, Final>$ be the symbolic encoding of $\UCW_{\psi}^k$.  The simple game to solve now becomes:

\[
\mathcal{H} = (V_H, D_H, \cont_H, \envi_H, \Psi),
\]
where
\begin{itemize}
\item $V_H$ := $V \union C$ , where $C = \{ c_0, c_1, . ..  c_{|Q| -1}\}$.
\item $D_H$ := $D \union D_C$ where  $D_C: C \rightarrow \{0, 1, 2,  k+1\}$
\item $\cont_H$ := $\cont \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$C$
\item $\envi_H$ := $\envi \wedge Aut$ is constraint over $V_H \union V_H' \union \{q,q'\}$  representing the moves of Player~$E$
  \item $\Psi$ := $G(Final)$
\end{itemize}

We can now solve this game using Algorithm \ref{proc: gensys-safety} mentioned in Section \ref{sec:simple-games}. 

Similarly,  in lines 75 -80, we check if environment has a strategy for $\neg \psi$.  If $<Aut, Final>$ is the symbolic encoding of of $\UCW_{\neg \psi}^k$, then the resulting game is:

\[
\mathcal{H} = (V_H, D_H, \envi_H, \cont_H, \Psi)
\]

where,  the definitions for each entry in the tuple is same as above.

\Stanly {This section needs to be better phrased}
For an increasing value of $k>=0$, we run both environment and controller strategies in parallel,  until $W_L == W_U$ or timeout.

We can now plug in $Con(V, V')$, $Env(V, V')$, and $Aut(q, V, q')$ into one of our two fixedpoint approaches to synthesize a controller to the above solution. Both approaches rely on a conversion from $Aut(q,V,q')$ to a $k$-safety game to check for $k$ realizability. If a solution is not found for a given value of $k$, we search for a higher value of $k$. Moreover, since the game is determined, we can also check for the realizability of $Env(V, V')$ in parallel and stop when one of the two says realizable. The advantage of both our approaches is that we do not determinize to a k-safety automaton manually. We encode constraints that reason over the determinized k-automaton during the fixedpoint computation itself, eliminating the need for explicit determinization. In the second approach, we optimize the first approach by using antichains to represent the state space compactly. In Section \ref{sec:otf}, we introduce the On-The-Fly determinization approach where explicit determinization is avoided and in Section \ref{sec:antichain}, we optimize the OTF approach using antichains to effectively make use of the state space.




\Stanly{Done:
  \begin{itemize}
  \item Describe representing automata symbolically
  \item Describe product game (symbolic)
  \item Describe UCW approach at high-level, refer to next
    sec/sections for details of OTF and Antichains.
  \end{itemize}}


==> overview.tex <==
\section{Overview of our Approach}
\label{sec:overview}


